Nerfels: Renderable Neural Codes for Improved Camera Pose Estimation

This paper presents a framework that combines traditional keypoint-based camera pose optimization with an invertible neural rendering mechanism. Our proposed 3D scene representation, Nerfels, is locally dense yet globally sparse. As opposed to existing invertible neural rendering systems which overfit a model to the entire scene, we adopt a feature-driven approach for representing scene-agnostic, local 3D patches with renderable codes. By modelling a scene only where local features are detected, our framework effectively generalizes to unseen local regions in the scene via an optimizable code conditioning mechanism in the neural renderer, all while maintaining the low memory footprint of a sparse 3D map representation. Our model can be incorporated to existing state-of-the-art hand-crafted and learned local feature pose estimators, yielding improved performance when evaluating on ScanNet for wide camera baseline scenarios.

==> egbib.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@inproceedings{mildenhall2020nerf,
  title={Nerf: Representing scenes as neural radiance fields for view synthesis},
  author={Mildenhall, Ben and Srinivasan, Pratul P and Tancik, Matthew and Barron, Jonathan T and Ramamoorthi, Ravi and Ng, Ren},
  booktitle={European Conference on Computer Vision},
  pages={405--421},
  year={2020},
  organization={Springer}
}

@article{yen2020inerf,
  title={iNeRF: Inverting Neural Radiance Fields for Pose Estimation},
  author={Yen-Chen, Lin and Florence, Pete and Barron, Jonathan T and Rodriguez, Alberto and Isola, Phillip and Lin, Tsung-Yi},
  journal={arXiv preprint arXiv:2012.05877},
  year={2020}
}

@inproceedings{schoenberger2016sfm,
    author={Sch\"{o}nberger, Johannes Lutz and Frahm, Jan-Michael},
    title={Structure-from-Motion Revisited},
    booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
    year={2016},
}

@inproceedings{schoenberger2016mvs,
    author={Sch\"{o}nberger, Johannes Lutz and Zheng, Enliang and Pollefeys, Marc and Frahm, Jan-Michael},
    title={Pixelwise View Selection for Unstructured Multi-View Stereo},
    booktitle={European Conference on Computer Vision (ECCV)},
    year={2016},
}

@article{tancik2020fourier,
  title={Fourier features let networks learn high frequency functions in low dimensional domains},
  author={Tancik, Matthew and Srinivasan, Pratul P and Mildenhall, Ben and Fridovich-Keil, Sara and Raghavan, Nithin and Singhal, Utkarsh and Ramamoorthi, Ravi and Barron, Jonathan T and Ng, Ren},
  journal={arXiv preprint arXiv:2006.10739},
  year={2020}
}

@article{lepetit2009epnp,
  title={Epnp: An accurate o (n) solution to the pnp problem},
  author={Lepetit, Vincent and Moreno-Noguer, Francesc and Fua, Pascal},
  journal={International journal of computer vision},
  volume={81},
  number={2},
  pages={155},
  year={2009},
  publisher={Springer}
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={8026--8037},
  year={2019}
}

@inproceedings{mccormac2017scenenet,
  title={Scenenet rgb-d: Can 5m synthetic images beat generic imagenet pre-training on indoor segmentation?},
  author={McCormac, John and Handa, Ankur and Leutenegger, Stefan and Davison, Andrew J},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2678--2687},
  year={2017}
}

@inproceedings{dai2017scannet,
  title={Scannet: Richly-annotated 3d reconstructions of indoor scenes},
  author={Dai, Angela and Chang, Angel X and Savva, Manolis and Halber, Maciej and Funkhouser, Thomas and Nie{\ss}ner, Matthias},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={5828--5839},
  year={2017}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{lowe2004distinctive,
  title={Distinctive image features from scale-invariant keypoints},
  author={Lowe, David G},
  journal={International journal of computer vision},
  volume={60},
  number={2},
  pages={91--110},
  year={2004},
  publisher={Springer}
}

@article{cadena2016past,
  title={Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age},
  author={Cadena, Cesar and Carlone, Luca and Carrillo, Henry and Latif, Yasir and Scaramuzza, Davide and Neira, Jos{\'e} and Reid, Ian and Leonard, John J},
  journal={IEEE Transactions on robotics},
  volume={32},
  number={6},
  pages={1309--1332},
  year={2016},
}

@conference {pfister2000,
    title={Surfels-Surface Elements as Rendering Primitives},
    author={H. Pfister and M. Zwicker and J. van Baar and M. Gross},
    booktitle={ACM Transactions on Graphics (Proc. ACM SIGGRAPH)},
    year={2000},
    month={7/2000},
    pages={335--342}
}

@INPROCEEDINGS{Lucas81,
    author = {Bruce D. Lucas and Takeo Kanade},
    title = {An iterative image registration technique with an application to stereo vision},
    booktitle = {In IJCAI81},
    year = {1981},
    pages = {674--679}
}

@InProceedings{agarwal2010,
author = {Agarwal, Sameer and Snavely, Noah and Seitz, Steven M. and Szeliski, Rick},
title = {Bundle Adjustment in the Large},
booktitle = {ECCV},
year = {2010},
}

@article{mur2015,
  title={{ORB-SLAM}: a versatile and accurate monocular {SLAM} system},
  author={Mur-Artal, Raul and Montiel, Jose and Tardos, Juan D},
  journal={IEEE Transactions on Robotics},
  year={2015},
  publisher={IEEE}
}

@INPROCEEDINGS{nister04,
    author = {David Nistér and Oleg Naroditsky and James Bergen},
    title = {Visual odometry},
    booktitle = {},
    year = {2004},
    pages = {652--659}
}

@article{ravi2020pytorch3d,
    author = {Nikhila Ravi and Jeremy Reizenstein and David Novotny and Taylor Gordon
                  and Wan-Yen Lo and Justin Johnson and Georgia Gkioxari},
    title = {Accelerating 3D Deep Learning with PyTorch3D},
    journal = {arXiv:2007.08501},
    year = {2020},
}

@InProceedings{Dusmanu2019CVPR,
    author = {Dusmanu, Mihai and Rocco, Ignacio and Pajdla, Tomas and Pollefeys, Marc and Sivic, Josef and Torii, Akihiko and Sattler, Torsten},
    title = {{D2-Net: A Trainable CNN for Joint Detection and Description of Local Features}},
    booktitle = {Proceedings of the 2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition},
    year = {2019},
}

@inproceedings{detone2018superpoint,
  title={Superpoint: Self-supervised interest point detection and description},
  author={DeTone, Daniel and Malisiewicz, Tomasz and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition workshops},
  pages={224--236},
  year={2018}
}

@inproceedings{sarlin2020superglue,
  title={Superglue: Learning feature matching with graph neural networks},
  author={Sarlin, Paul-Edouard and DeTone, Daniel and Malisiewicz, Tomasz and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={4938--4947},
  year={2020}
}

@inproceedings{dusmanu2020multi,
  title={Multi-View optimization of local feature geometry},
  author={Dusmanu, Mihai and Sch{\"o}nberger, Johannes L and Pollefeys, Marc},
  booktitle={European Conference on Computer Vision},
  pages={670--686},
  year={2020},
  organization={Springer}
}

@inproceedings{whelan15, 
    AUTHOR    = {Thomas Whelan AND Stefan Leutenegger AND Renato Salas Moreno AND Ben Glocker AND Andrew Davison}, 
    TITLE     = {ElasticFusion: Dense SLAM Without A Pose Graph}, 
    BOOKTITLE = {Proceedings of Robotics: Science and Systems}, 
    YEAR      = {2015}, 
    ADDRESS   = {Rome, Italy}, 
    MONTH     = {July},
    DOI       = {10.15607/RSS.2015.XI.001} 
}


@inproceedings{remata2021,
  author    = {Konstantinos Rematas and
               Ricardo Martin{-}Brualla and
               Vittorio Ferrari},
  title     = {ShaRF: Shape-conditioned Radiance Fields from a Single View},
  journal   = {CoRR},
  volume    = {abs/2102.08860},
  year      = {2021},
}


@inproceedings{Schwarz2020,
  title = {GRAF: Generative Radiance Fields for 3D-Aware Image Synthesis},
  author = {Schwarz, Katja and Liao, Yiyi and Niemeyer, Michael and Geiger, Andreas},
  booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
  year = {2020}
}

@inproceedings{bloesch2018,
 title = {CodeSLAM—learning a compact, optimisable representation for dense visual SLAM},
 author = {M Bloesch and J Czarnowski and R Clark and S Leutenegger and AJ Davison},
 booktitle = {Proceedings of the IEEE conference on computer vision and pattern recognition},
 pages = {2560--2568},
 year = {2018},
}

@inproceedings{engel2014lsd,
  title={LSD-SLAM: Large-Scale Direct Monocular SLAM},
  author={Jakob Engel and Thomas Sch{\"o}ps and D. Cremers},
  booktitle={ECCV},
  year={2014}
}

@article{engel2018dso,
  title={Direct Sparse Odometry},
  author={Jakob Engel and V. Koltun and D. Cremers},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2018},
  volume={40},
  pages={611-625}
}

@inproceedings{tang2018ba,
  author = {Tang, Chengzhou and Tan, Ping},
  title = {{{BA-Net:} Dense Bundle Adjustment Network}},
  year = 2019,
  booktitle = {ICLR}
}

@inproceedings{zhou2018deeptam,
  title={Deeptam: Deep tracking and mapping},
  author={Zhou, Huizhong and Ummenhofer, Benjamin and Brox, Thomas},
  booktitle={ECCV},
  year={2018}
}

@article{park2019,
  title={DeepSDF: Learning Continuous Signed Distance Functions for Shape Representation},
  author={Jeong Joon Park and Peter R. Florence and J. Straub and Richard A. Newcombe and S. Lovegrove},
  journal={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2019},
  pages={165-174}
}

@inproceedings{wang2021ibrnet,
  author    = {Wang, Qianqian and Wang, Zhicheng and Genova, Kyle and Srinivasan, Pratul and Zhou, Howard  and Barron, Jonathan T. and Martin-Brualla, Ricardo and Snavely, Noah and Funkhouser, Thomas},
  title     = {IBRNet: Learning Multi-View Image-Based Rendering},
  booktitle = {CVPR},
  year      = {2021}
}

@article{lin2020iNeRF,
  title={iNeRF: Inverting Neural Radiance Fields for Pose Estimation},
  author={Yen-Chen Lin and Peter R. Florence and J. T. Barron and Alberto Rodriguez and Phillip Isola and Tsung-Yi Lin},
  journal={ArXiv},
  year={2020},
  volume={abs/2012.05877}
}

@inproceedings{lin2021barf,
  title={BARF: Bundle-Adjusting Neural Radiance Fields},
  author={Lin, Chen-Hsuan and Ma, Wei-Chiu and Torralba, Antonio and Lucey, Simon},
  booktitle={IEEE International Conference on Computer Vision ({ICCV})},
  year={2021}
}

@inproceedings{sucar2020,
    title={{NodeSLAM}: Neural Object Descriptors for Multi-View Shape Reconstruction},
    author={Edgar Sucar and Kentaro Wada and Andrew Davison},
    booktitle={Proceedings of the International Conference on 3D Vision ({3DV})},
    year={2020},
}
  
@inproceedings{runz2020frodo,
  title={FroDO: From Detections to 3D Objects},
  author={Runz, Martin and Li, Kejie and Tang, Meng and Ma, Lingni and Kong, Chen and Schmidt, Tanner and Reid, Ian and Agapito, Lourdes and Straub, Julian and Lovegrove, Steven and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14720--14729},
  year={2020}
}

@InProceedings{genova2020,
author = {Genova, Kyle and Cole, Forrester and Sud, Avneesh and Sarna, Aaron and Funkhouser, Thomas},
title = {Local Deep Implicit Functions for 3D Shape},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2020}
}

@InProceedings{chabra2020,
author = {Chabra, Rohan and Lenssen, Jan E. and Ilg, Eddy and Schmidt, Tanner and Straub, Julian and Lovegrove, Steven and Newcombe, Richard},
    booktitle={European Conference on Computer Vision (ECCV)},
    year={2020},
}

@inproceedings{jiang2020,
  title = {Local Implicit Grid Representations for 3D Scenes},
  author = {Chiyu Max Jiang and Avneesh Sud and Ameesh Makadia and Jingwei Huang and Matthias Nießner and Thomas Funkhouser},
  booktitle = {Proceedings IEEE Conf. on Computer Vision and Pattern Recognition (CVPR)},
  year = {2020}
}


@inproceedings{reiser2021,
  author    = {Christian Reiser and
               Songyou Peng and
               Yiyi Liao and
               Andreas Geiger},
  title     = {KiloNeRF: Speeding up Neural Radiance Fields with Thousands of Tiny
               MLPs},
  booktitle   = {IEEE International Conference on Computer Vision ({ICCV})},
  year      = {2021},
}

@InProceedings{henriques2018,
author = {Henriques, João F. and Vedaldi, Andrea},
title = {MapNet: An Allocentric Spatial Memory for Mapping Environments},
booktitle = {Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2018}
}



@InProceedings{avraham2018,
author = {Gil Avraham and Yan Zuo and Thanuja Dharmasiri and Tom Drummond},
title = {EMPNet: Neural Localisation and Mapping Using Embedded Memory Points},
  booktitle   = {IEEE International Conference on Computer Vision ({ICCV})},
  year      = {2018},
}

@inproceedings{klein2007parallel,
  title={Parallel tracking and mapping for small AR workspaces},
  author={Klein, Georg and Murray, David},
  booktitle={2007 6th IEEE and ACM international symposium on mixed and augmented reality},
  pages={225--234},
  year={2007},
  organization={IEEE}
}

@article{scaramuzza2011visual,
  title={Visual odometry [tutorial]},
  author={Scaramuzza, Davide and Fraundorfer, Friedrich},
  journal={IEEE robotics \& automation magazine},
  volume={18},
  number={4},
  pages={80--92},
  year={2011},
  publisher={IEEE}
}

@article{davison2007,
  author={Davison, Andrew J. and Reid, Ian D. and Molton, Nicholas D. and Stasse, Olivier},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={MonoSLAM: Real-Time Single Camera SLAM}, 
  year={2007},
  volume={29},
  number={6},
  pages={1052-1067},
  doi={10.1109/TPAMI.2007.1049}
}
  
  
  @article{agarwal2011,
title	= {Building Rome in a day},
author	= {Sameer Agarwal and Yasutaka Furukawa and Noah Snavely and Ian Simon and Brian Curless and Steven M. Seitz and Rick Szeliski},
year	= {2011},
journal	= {Communications of the ACM},
pages	= {105--112},
volume	= {54}
}

@inproceedings{harris1988,
  title={A combined corner and edge detector.},
  author={Harris, Chris and Stephens, Mike},
  booktitle={Alvey vision conference},
  volume={15},
  number={50},
  pages={10--5244},
  year={1988},
  organization={Manchester, UK}
}

@article{Mescheder2019OccupancyNL,
  title={Occupancy Networks: Learning 3D Reconstruction in Function Space},
  author={Lars M. Mescheder and Michael Oechsle and Michael Niemeyer and S. Nowozin and Andreas Geiger},
  journal={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2019},
  pages={4455-4465}
}

@article{wang2021nerfmm,
  title={Ne{RF}$--$: Neural Radiance Fields Without Known Camera Parameters},
  author={Zirui Wang and Shangzhe Wu and Weidi Xie and Min Chen and Victor Adrian Prisacariu},
  journal={arXiv preprint arXiv:2102.07064},
  year={2021}
}

@inproceedings{newcombe2011dtam,
  author = {Newcombe, Richard A. and Lovegrove, Steven and Davison, Andrew J.},
  booktitle   = {IEEE International Conference on Computer Vision ({ICCV})},
  title = {DTAM: Dense tracking and mapping in real-time.},
  year = 2011
}

@inproceedings{zhou2017,
  author    = {Tinghui Zhou and
               Matthew Brown and
               Noah Snavely and
               David G. Lowe},
    title={Unsupervised Learning of Depth and Ego-Motion from Video},
    booktitle={Conference on Computer Vision and Pattern Recognition (CVPR)},
    year={2017}
}

@article{henry2012,
author = {Peter Henry and Michael Krainin and Evan Herbst and Xiaofeng Ren and Dieter Fox},
title ={RGB-D mapping: Using Kinect-style depth cameras for dense 3D modeling of indoor environments},
journal = {The International Journal of Robotics Research},
year = {2012},
}

@inproceedings{newcombe2011kinect,
  author = {Newcombe, Richard A. and Izadi, Shahram and Hilliges, Otmar and Molyneaux, David and Kim, David and Davison, Andrew J. and Kohli, Pushmeet and Shotton, Jamie and Hodges, Steve and Fitzgibbon, Andrew W.},
  title = {KinectFusion: Real-time dense surface mapping and tracking.},
  year = 2011
}

@article{Kendall2015PoseNetAC,
  title={PoseNet: A Convolutional Network for Real-Time 6-DOF Camera Relocalization},
  author={Alex Kendall and M. Grimes and R. Cipolla},
  journal={2015 IEEE International Conference on Computer Vision (ICCV)},
  booktitle={ICCV},
  year={2015},
  pages={2938-2946}
}

  @inproceedings{sucar2021,
    title={{iMAP}: Implicit Mapping and Positioning in Real-Time},
    author={Edgar Sucar and Shikun Liu and Joseph Ortiz and Andrew Davison},
    booktitle={arXiv preprint arXiv:2103.12352},
    year={2021},
  }
  
@inproceedings{sitzmann2019siren,
author = {Sitzmann, Vincent
          and Martel, Julien N.P.
          and Bergman, Alexander W.
          and Lindell, David B.
          and Wetzstein, Gordon},
title = {Implicit Neural Representations
          with Periodic Activation Functions},
booktitle = {Proc. NeurIPS},
year={2020}
}

@inproceedings{balntas2018relocnet,
  title={RelocNet: Continuous Metric Learning Relocalisation Using Neural Nets},
  author={Vassileios Balntas and Shuda Li and V. Prisacariu},
  booktitle={ECCV},
  year={2018}
}

@inproceedings{wang18deepvo,
  title={End-to-End, Sequence-to-Sequence Probabilistic Visual Odometry through Deep Neural Networks},
  author={Sen Wang and Ronald Clark and Hongkai Wen and Niki Trigoni},
  booktitle={Journal of Robotics Research (IJRR)},
  year={2018}
}


@misc{ceres-solver,
  author = "Sameer Agarwal and Keir Mierle and Others",
  title = "Ceres Solver",
  howpublished = "\url{http://ceres-solver.org}",
}

@article{lassner2020pulsar,
    author = {Christoph Lassner and Michael Zollh\"ofer},
    title = {Pulsar: Efficient Sphere-based Neural Rendering},
    journal = {arXiv:2004.07484},
    year = {2020},
}

@inproceedings{nardi2015introducing,
  title={Introducing SLAMBench, a performance and accuracy benchmarking methodology for SLAM},
  author={Nardi, Luigi and Bodin, Bruno and Zia, M Zeeshan and Mawer, John and Nisbet, Andy and Kelly, Paul HJ and Davison, Andrew J and Luj{\'a}n, Mikel and O'Boyle, Michael FP and Riley, Graham and others},
  booktitle={2015 IEEE international conference on robotics and automation (ICRA)},
  pages={5783--5790},
  year={2015},
  organization={IEEE}
}

@INPROCEEDINGS{reiser2021ICCV,
  author = {Christian Reiser and Songyou Peng and Yiyi Liao and Andreas Geiger},
  title = {KiloNeRF: Speeding up Neural Radiance Fields with Thousands of Tiny MLPs},
  booktitle = {International Conference on Computer Vision (ICCV)},
  year = {2021}
}

@article{garbin2021,
  author    = {Stephan J. Garbin and
               Marek Kowalski and
               Matthew Johnson and
               Jamie Shotton and
               Julien P. C. Valentin},
  title     = {FastNeRF: High-Fidelity Neural Rendering at 200FPS},
  journal   = {arXiv:2103.10380},
  year      = {2021},
}

@article{hedman2021snerg,
    title={Baking Neural Radiance Fields for
           Real-Time View Synthesis},
    author={Peter Hedman and Pratul P. Srinivasan and
            Ben Mildenhall and Jonathan T. Barron and
            Paul Debevec},
    journal={ICCV},
    year={2021}
}
